First search for ultralight dark matter with a space-based gravitational-wave antenna: LISA Pathfinder

We present here results from the first-ever search for dark photon dark matter that could have coupled to baryons in LISA Pathfinder, the technology demonstrator for a space-based gravitational-wave antenna. After analyzing approximately three months of data taken by LISA Pathfinder in the frequency range $[2\times 10^{-5},5]$ Hz, corresponding to dark photon masses of $[8\times 10^{-20},2\times 10^{-14}]$ eV/$c^2$, we find no evidence of a dark-matter signal, and set upper limits on the strength of the dark photon/baryon coupling. To perform this search, we leveraged methods that search for quasi-monochromatic gravitational-wave signals in ground-based interferometers, and are robust against non-Gaussianities and gaps in the data. Our work therefore represents a proof-of-concept test of search methods in LISA to find persistent, quasi-monochromatic signals, and shows our ability to handle non-Guassian artifacts and gaps while maintaining good sensitivity compared to the optimal matched filter. The results also indicate that these methods can be powerful tools in LISA to not only find dark matter, but also look for other persistent signals from e.g. intermediate-mass black hole inspirals and galactic white dwarf binaries.

==> last_cands_rest.tex <==
\begin{table}
\begin{tabular}{|c|c|}
\hline 
frequency (Hz) & SNR \\ 
\hline 
0.474766 & 8.57 \\ 
1.213422 & 8.50 \\ 
2.584182 & 8.26 \\ 
\hline 
\end{tabular}
\caption{\label{tab:cands} Remaining candidates from the fully coherent, high-frequency search that appeared in at least two the datasets analyzed. We note that these candidates did not appear in all segments analyzed, as we would expect for a true dark photon signal; thus, we veto them. }
\end{table}

==> table_segs_dur_tfft_temp.tex <==
\begin{table}
\begin{tabular}{|c|c|c|c|c|}
\hline 
number & date & duration (days) & $T_{\rm FFT}$ (s) & Temp (C) \\ 
\hline 
1 & 2016-03-$21$ & 5.08 & 16384 & 22 \\ 
2 & 2016-04-$04$ & 9.33 & 16384 & 22 \\ 
3 & 2016-07-$24$ & 5.29 & 4096 & 22 \\ 
4 & 2016-11-$16$ & 9.82 & 8192 & 22 \\ 
5 & 2016-12-$26$ & 17.86 & 8192 & 22 \\ 
6 & 2017-02-$14$ & 13.33 & 8192 & 11 \\ 
7 & 2017-05-$29$ & 7.04 & 131072 & 22 \\ 
8 & 2017-06-$08$ & 8.4 & 262144 & 22 \\ 
\hline 
\end{tabular}
\caption{\label{tab:segs} Data segments considered in this search obtained from \cite{lpfarchive}. Segment \# 6 is treated as a separate dataset here: we perform coincidences of the other seven datasets with segment \# 6 in order to reduce the number of outliers.}
\end{table}
